Pattern Matching with Edits in $\tilde{O}(n+k^3\cdot n/m)$ Time

Given a pattern $P$ of length $m$, a text $T$ of length $n$, and a threshold $k$, the Pattern Matching with Edits problem asks whether $T$ contains a substring that can be transformed into $P$ using at most $k$ character insertions, deletions, and substitutions. The classic $O(nm)$- and $O(nk)$-time algorithms of Sellers [J. Algorithms'80] and Landau and Vishkin [STOC'86, J. Algorithms'89] are near-optimal for $k=\Theta(m)$ under the Orthogonal Vectors Hypothesis. For small $k$, Cole and Hariharan [SODA'98, SICOMP'02] achieved $O(n+k^4\cdot n/m)$ time, and Charalampopoulos, Kociumaka, and Wellnitz (CKW) [FOCS'22] improved this to $O(n+k^{3.5}\log k\cdot n/m)$, essentially halfway to the $O(n+k^3\cdot n/m)$ bound conjectured by Cole and Hariharan. This work confirms the conjecture up to a polylogarithmic factor with an $O(n+k^3\log^2 k\cdot n/m)$-time algorithm. Working in the PILLAR model [CKW; FOCS'20], which accesses strings only through a few basic operations, it extends to grammar-compressed, dynamic, quantum, and small-space read-only settings. It also closes, up to the $\log^2 k$ factor, the longstanding gap to certain aperiodic patterns, for which Cole and Hariharan achieved $O(n+k^3\cdot n/m)$ time. The alternative approach of CKW [FOCS'20] leaves one bottleneck, which the general case reduces to: $P$ and $T$ are close to periodic strings with a common period. This case amounts to many min-plus products of distance matrices, each consisting of long runs of one fixed matrix separated by $O(k)$ other matrices. We collapse every long run into a single matrix and show that this preserves the distances that determine the occurrences unless the periodicity-breaking parts of $P$ and $T$ interact strongly. Our main structural result, a planar variation theorem, confines the exact computations needed in the remaining cases to narrow regions of the alignment graph.

==> settings.tex <==

\makeatletter
\newcommand{\refcheckize}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[1]{%
    \csname @@\string#1\endcsname{##1}\@for\@temp:=##1\do{\wrtusdrf{\@temp}\wrtusdrf{{\@temp}}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\newcommand{\refcheckizetwo}[1]{%
  \expandafter\let\csname @@\string#1\endcsname#1%
  \expandafter\DeclareRobustCommand\csname relax\string#1\endcsname[2]{%
    \csname @@\string#1\endcsname{##1}{##2}\wrtusdrf{##1}\wrtusdrf{{##1}}\wrtusdrf{##2}\wrtusdrf{{##2}}}%
  \expandafter\let\expandafter#1\csname relax\string#1\endcsname
}
\makeatother

\refcheckize{\cref}
\refcheckize{\Cref}
\refcheckizetwo{\crefrange}
\refcheckizetwo{\Crefrange}

\makeatletter
\renewcommand\thmt@autorefsetup{\@xa\def\csname\thmt@envname autorefname\@xa\endcsname\@xa{\thmt@thmname}}
\makeatother

\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{mtheorem}{Main Theorem}
\crefname{fact}{Fact}{Facts}
\crefname{mtheorem}{Main Theorem}{Main Theorems}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheoremstyle{claimstyle}{\topsep}{\topsep}{\itshape}{}{\scshape}{.}{5pt plus 1pt minus 1pt}{}
\theoremstyle{claimstyle}
\newtheorem{claim}[theorem]{Claim}
\crefname{claim}{Claim}{Claims}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}

\theoremstyle{plain}
\newtheorem{theoremq}[theorem]{Theorem}
\newtheorem{lemmaq}[theorem]{Lemma}
\newtheorem{corollaryq}[theorem]{Corollary}
\crefname{theoremq}{Theorem}{Theorems}
\Crefname{theoremq}{Theorem}{Theorems}
\crefname{lemmaq}{Lemma}{Lemmas}
\Crefname{lemmaq}{Lemma}{Lemmas}
\crefname{corollaryq}{Corollary}{Corollaries}
\Crefname{corollaryq}{Corollary}{Corollaries}

\newcommand{\claimqedsymbol}{\ensuremath{\lhd}}
\newenvironment{claimproof}[1][\proofname]
  {\renewcommand{\qedsymbol}{\claimqedsymbol}\begin{proof}[\normalfont\scshape #1]}
  {\end{proof}}
\newcommand{\claimqedhere}{\qedhere}

\newcommand{\lipicsEnd}{}

\NewDocumentCommand{\dglabel}{s t^ t" m O{} D(){}}{\label{#4}}

\AddToHook{env/theorem/begin}{\crefalias{section}{theorem}}
\AddToHook{env/corollary/begin}{\crefalias{theorem}{corollary}}
\AddToHook{env/lemma/begin}{\crefalias{theorem}{lemma}}
\AddToHook{env/fact/begin}{\crefalias{theorem}{fact}}
\AddToHook{env/observation/begin}{\crefalias{theorem}{observation}}
\AddToHook{env/proposition/begin}{\crefalias{theorem}{proposition}}
\AddToHook{env/definition/begin}{\crefalias{theorem}{definition}}
\AddToHook{env/claim/begin}{\crefalias{theorem}{claim}}
\AddToHook{env/theoremq/begin}{\crefalias{section}{theorem}}
\AddToHook{env/lemmaq/begin}{\crefalias{theorem}{lemma}}
\AddToHook{env/corollaryq/begin}{\crefalias{theorem}{corollary}}
\AddToHook{env/remark/begin}{\crefalias{theorem}{remark}}
\AddToHook{env/example/begin}{\crefalias{theorem}{example}}

\def\theHtheorem{\theHsection.\arabic{theorem}}
\def\theHcorollary{\theHsection.\arabic{theorem}}
\def\theHlemma{\theHsection.\arabic{theorem}}
\def\theHfact{\theHsection.\arabic{theorem}}
\def\theHproposition{\theHsection.\arabic{theorem}}
\def\theHdefinition{\theHsection.\arabic{theorem}}
\def\theHclaim{\theHsection.\arabic{theorem}}
\def\theHtheoremq{\theHsection.\arabic{theorem}}
\def\theHlemmaq{\theHsection.\arabic{theorem}}
\def\theHcorollaryq{\theHsection.\arabic{theorem}}
\def\theHremark{\theHsection.\arabic{theorem}}
\def\theHexample{\theHsection.\arabic{theorem}}

\crefname{algocf}{Algorithm}{Algorithms}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{algocfline}{Line}{Lines}
\Crefname{algocfline}{Line}{Lines}

\definecolor{mypink}{RGB}{199, 21, 133}
\hypersetup{
  colorlinks,
  urlcolor = blue,
  linkcolor = mypink,
  citecolor = blue
}

\setul{2pt}{0.6pt}

\setlength{\FrameSep}{1.5ex}

\setlength{\OuterFrameSep}{\topsep}
\renewenvironment{framed}
  {\par\addvspace{\OuterFrameSep}%
   \ifdefined\nolinenumbers\nolinenumbers\fi
   \noindent\begin{minipage}{\linewidth}%
   \MakeFramed{\advance\hsize-\width\FrameRestore}}
  {\endMakeFramed\end{minipage}\par\addvspace{\OuterFrameSep}}

\setlist[enumerate]{nosep, topsep=1ex}
\setlist[itemize]{nosep, topsep=1ex}
\setlist[description]{nosep,topsep=1ex}

\allowdisplaybreaks

\lineskiplimit=-5pt

\let\oldabstract\abstract
\let\oldendabstract\endabstract
\makeatletter
\renewenvironment{abstract}
{\renewenvironment{quotation}%
  {\list{}{\addtolength{\leftmargin}{1.9em}%
    \listparindent 1.5em%
     \itemindent    \listparindent%
     \rightmargin   \leftmargin%
     \parsep        \z@ \@plus\p@}%
     \item\relax}%
  {\endlist}%
\oldabstract}
{\oldendabstract}
\makeatother

\let\OLDthebibliography\thebibliography
  \renewcommand\thebibliography[1]{
  \OLDthebibliography{#1}
  \setlength{\parskip}{0pt}
  \setlength{\itemsep}{0pt plus 0.3ex}
}

\newenvironment{bfdescription}
  {\begin{description}[style=sameline,itemsep=1ex,font={\normalfont\bf}]}
  {\end{description}\vspace{-1.2ex}}

\renewcommand*\descriptionlabel[1]{\hspace\labelsep\normalfont\itshape #1}

\setlength{\emergencystretch}{1.5em}

\definecolor{color1}{HTML}{648FFF} %
\definecolor{color2}{HTML}{785EF0} %
\definecolor{color3}{HTML}{DC267F} %
\definecolor{color4}{HTML}{FE6100} %
\definecolor{color5}{HTML}{FFB000} %
\colorlet{c1}{color1!60!black}
\colorlet{c2}{color2!60!black}
\colorlet{c3}{color3!60!black}
\colorlet{c4}{color4!60!black}
\colorlet{c5}{color5!60!black}

\providecommand{\probname}[1]{\text{\sc #1}}
\crefname{problem}{the}{the}
\Crefname{problem}{The}{The}
\creflabelformat{problem}{#2#1#3 problem}
\makeatletter
\ExplSyntaxOn
\newcounter{@@p}
\clist_new:N \g__problem_pitem_iname_clist
\clist_new:N \g__problem_pitem_itext_clist
\NewDocumentEnvironment{problem}{o m}{%
  \newcounter{@@p@\the@@p}%
  \crefalias{@@p@\the@@p}{problem}%
  \IfValueTF{#1}
    {\expandafter\gdef\csname the@@p@\the@@p\endcsname{{\protect #1}}}
    {\expandafter\gdef\csname the@@p@\the@@p\endcsname{{\protect #2}}}%
  \setcounter{@@p@\the@@p}{\the@@p}\refstepcounter{@@p@\the@@p}%
  \stepcounter{@@p}%
  \clist_gclear:N \g__problem_pitem_iname_clist
  \clist_gclear:N \g__problem_pitem_itext_clist
  \NewDocumentCommand{\PItem}{m m}{%
    \clist_gput_right:Nn \g__problem_pitem_iname_clist {{##1}}%
    \clist_gput_right:Nn \g__problem_pitem_itext_clist {{##2}}%
  }%
  \NewDocumentCommand{\PInput}{m}{\PItem{Input}{##1}}%
  \NewDocumentCommand{\POutput}{m}{\PItem{Output}{##1}}%
  \NewDocumentCommand{\PTask}{m}{\PItem{Task}{##1}}%
  \NewDocumentCommand{\PParameter}{m}{\PItem{Parameter}{##1}}%
}{%
  \begin{framed}
    \noindent\probname{#2}
    \begin{bfdescription}
      \clist_set_eq:NN \l_tmpa_clist \g__problem_pitem_iname_clist
      \clist_set_eq:NN \l_tmpb_clist \g__problem_pitem_itext_clist
      \bool_until_do:nn {\clist_if_empty_p:N \l_tmpa_clist}{
        \clist_pop:NN \l_tmpa_clist \l_tmpa_tl
        \clist_pop:NN \l_tmpb_clist \l_tmpb_tl
        \item[\l_tmpa_tl{}:]~\l_tmpb_tl
      }
    \end{bfdescription}
  \end{framed}
}
\ExplSyntaxOff
\makeatother

